Towards the Use of Slice-based Cohesion Metrics with Learning Analytics to Assess Programming Skills

In programming education, it makes a difference whether you are dealing with beginners or advanced students. As our future students will become even more tech-savvy, it is necessary to assess programming skills appropriately and quickly to protect them from boredom and optimally support the learning process. In this work, we advocate for the use of slice-based cohesion metrics to assess the process of program construction in a learning analytics setting. We argue that semantically related parts during program construction are an essential part of programming skills. Therefore, we propose using cohesion metrics on the level of variables to identify programmers' trains of thought based on the cohesion of semantically related parts during program construction.

==> data/method1-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{r}
 \\
\multicolumn{1}{l}{\texttt{void convertBinArr(int[] bN)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} double dec=0;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} String hex="";}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} for(int i = 0; i$<$bN.length; i++)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} if(bN[i]$==$1)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}iii\color{black} dec+=Math.pow(2,i);}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} $\}$  $\}$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(dec);}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(hex); $\}$}} \\
 \\
\end{tabular}%


==> data/method1-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{r}
 \\
\multicolumn{1}{l}{\texttt{void convertBinArr(int[] bN)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int sum=0;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int m = 1;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} for(int i=0;i$<$bN.length;i++)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} sum+=m*bN[i];}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} m*=2;  $\}$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(sum); $\}$}} \\
 \\
\end{tabular}%


==> data/method2-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{r}
 \\
\multicolumn{1}{l}{\texttt{void convertBinArr(int[] bN)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} double dec=0;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} String hex="";}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} double hD=0;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} for(int i = 0; i$<$bN.length; i++)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} if(bN[i]$==$1)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}iii\color{black} dec+=Math.pow(2,i);}} \\
\multicolumn{1}{l}{\texttt{\color{white}iii\color{black} if(i$<=$3)}} \\
\multicolumn{1}{l}{\texttt{\color{white}iiii\color{black} hD+=Math.pow(2,i);}} \\
\multicolumn{1}{l}{\texttt{\color{white}iii\color{black} if(i$>$3)}} \\
\multicolumn{1}{l}{\texttt{\color{white}iiii\color{black} hD+=Math.pow(2,i-4);}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} $\}$  $\}$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(dec);}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(hD); $\}$}} \\
 \\
\end{tabular}%


==> data/method2-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{r}
 \\
\multicolumn{1}{l}{\texttt{void convertBinArr(int[] bN)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int sum=0;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int m = 1;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} for(int i=0;i$<$bN.length;i++)$\{$}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} sum+=m*bN[i];}} \\
\multicolumn{1}{l}{\texttt{\color{white}ii\color{black} m*=2;  $\}$}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} System.out.println(sum);}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int c1=sum/16;}} \\
\multicolumn{1}{l}{\texttt{\color{white}i\color{black} int c2=sum\%16; $\}$}} \\
 \\
\end{tabular}%


==> data/metrics-comparison-1.tex <==
\small

% Table generated by Excel2LaTeX from sheet 'comparison'
\begin{tabular}{l|ccccc}
\multicolumn{6}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{c 1/2}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\cmidrule{2-6}\textit{\textbf{bN}} & 1     & 1     & 1     & 1     & 1 \\
\textit{\textbf{c 1/2}} & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .651,  .651,  .651}.20 \\
\textit{\textbf{i}} & 1     & 1     & 1     & 1     & 1 \\
\textit{\textbf{m}} & 1     & 1     & 1     & 1     & .80 \\
\textit{\textbf{sum}} & 1     & 1     & 1     & 1     & 1 \\
\end{tabular}%



==> data/metrics-comparison-2.tex <==
\small

% Table generated by Excel2LaTeX from sheet 'comparison'
\begin{tabular}{l|cccc}
\multicolumn{5}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & 1     & 1     & 1     & 1 \\
\textit{\textbf{i}} & 1     & 1     & 1     & 1 \\
\textit{\textbf{m}} & 1     & 1     & 1     & .75 \\
\textit{\textbf{sum}} & 1     & 1     & 1     & 1 \\
\end{tabular}%



==> data/metrics-comparison-3.tex <==
\small

% Table generated by Excel2LaTeX from sheet 'comparison'
\begin{tabular}{l|cccccc}
\multicolumn{1}{r}{} & \multicolumn{6}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{hexD1}} & \textit{\textbf{hexD2}} & \textit{\textbf{i}} \\
\cmidrule{2-7}\textit{\textbf{bN}} & 1     & .67   & .67   & .67   & .67   & 1 \\
\textit{\textbf{dec}} & \cellcolor[rgb]{ .851,  .851,  .851}1 & \cellcolor[rgb]{ .851,  .851,  .851}1 & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .851,  .851,  .851}.67 \\
\textit{\textbf{hex}} & \cellcolor[rgb]{ .651,  .651,  .651}.50 & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .651,  .651,  .651}.50 & \cellcolor[rgb]{ .651,  .651,  .651}.50 & \cellcolor[rgb]{ .651,  .651,  .651}.50 & \cellcolor[rgb]{ .651,  .651,  .651}.44 \\
\textit{\textbf{hexD1}} & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .651,  .651,  .651}.67 & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ .651,  .651,  .651}.89 \\
\textit{\textbf{hexD2}} & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ 0,  0,  0}\textcolor[rgb]{ 1,  1,  1}{0} & \cellcolor[rgb]{ .651,  .651,  .651}.67 & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ .651,  .651,  .651}1 & \cellcolor[rgb]{ .651,  .651,  .651}.89 \\
\textit{\textbf{i}} & 1     & .67   & .67   & 1     & .67   & 1 \\
\end{tabular}%


==> data/metrics1-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{l|cccc}
\multicolumn{5}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{i}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .4,  .761,  .643}.67 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{dec}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{hex}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\multicolumn{1}{r}{} &       &       &       &  \\
\multicolumn{5}{c}{\textit{\textbf{PairOverlap (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{i}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{dec}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{hex}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\end{tabular}%



==> data/metrics1-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{l|cccc}
\multicolumn{5}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{m}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .4,  .761,  .643}.67 \\
\textit{\textbf{sum}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\end{tabular}%


==> data/metrics2-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{l|ccccc}
\multicolumn{6}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{hD}} & \textit{\textbf{i}} \\
\cmidrule{2-6}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .4,  .761,  .643}.67 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}.75 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{dec}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .4,  .761,  .643}.56 \\
\textit{\textbf{hex}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 \\
\textit{\textbf{hD}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}.89 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .4,  .761,  .643}.67 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\multicolumn{1}{r}{} &       &       &       &       &  \\
\multicolumn{1}{r}{} &       &       &       &       &  \\
\multicolumn{6}{c}{\textit{\textbf{PairOverlap (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{hD}} & \textit{\textbf{i}} \\
\cmidrule{2-6}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{dec}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{hex}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 \\
\textit{\textbf{hD}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\end{tabular}%


==> data/metrics2-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{l|ccccc}
\multicolumn{6}{c}{\textit{\textbf{PairCoverage (REF+DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{c 1/2}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\cmidrule{2-6}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{c 1/2}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .929,  .973,  .984}.20 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{m}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}.80 \\
\textit{\textbf{sum}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\end{tabular}%


==> data/metrics3-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}[b]{rrrrrr}
\multicolumn{6}{c}{\textit{\textbf{PairCoverage (REF)}}} \\
      & \multicolumn{1}{c}{\textit{\textbf{bN}}} & \multicolumn{1}{c}{\textit{\textbf{dec}}} & \multicolumn{1}{c}{\textit{\textbf{hex}}} & \multicolumn{1}{c}{\textit{\textbf{hD1/2}}} & \multicolumn{1}{c}{\textit{\textbf{i}}} \\
\cmidrule{2-6}\multicolumn{1}{l|}{\textit{\textbf{bN}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\multicolumn{1}{l|}{\textit{\textbf{dec}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} \\
\multicolumn{1}{l|}{\textit{\textbf{hex}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .698,  .886,  .886}.44} \\
\multicolumn{1}{l|}{\textit{\textbf{hD1}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}.88} \\
\multicolumn{1}{l|}{\textit{\textbf{hD2}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}.88} \\
\multicolumn{1}{l|}{\textit{\textbf{i}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
      &       &       &       &       &  \\
\multicolumn{6}{c}{\textit{\textbf{PairCoverage (DEF)}}} \\
      & \multicolumn{1}{c}{\textit{\textbf{bN}}} & \multicolumn{1}{c}{\textit{\textbf{dec}}} & \multicolumn{1}{c}{\textit{\textbf{hex}}} & \multicolumn{1}{c}{\textit{\textbf{hD1/2}}} & \multicolumn{1}{c}{\textit{\textbf{i}}} \\
\cmidrule{2-6}\multicolumn{1}{l|}{\textit{\textbf{bN}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\multicolumn{1}{l|}{\textit{\textbf{dec}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\multicolumn{1}{l|}{\textit{\textbf{hex}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} \\
\multicolumn{1}{l|}{\textit{\textbf{hD1}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\multicolumn{1}{l|}{\textit{\textbf{hD2}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\multicolumn{1}{l|}{\textit{\textbf{i}}} & \multicolumn{1}{c}{\cellcolor[rgb]{ .929,  .973,  .984}0} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .4,  .761,  .643}1/.50} & \multicolumn{1}{c}{\cellcolor[rgb]{ .137,  .545,  .271}1} \\
\end{tabular}%


==> data/metrics3-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
% Table generated by Excel2LaTeX from sheet '347'
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}[b]{l|cccc}
\multicolumn{5}{c}{\textit{\textbf{PairCoverage (REF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{mul}} & \textit{\textbf{sum}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{mul}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{sum}} & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\multicolumn{1}{r}{} &       &       &       &  \\
\multicolumn{5}{c}{\textit{\textbf{PairCoverage (DEF)}}} \\
\multicolumn{1}{r}{} & \textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{mul}} & \textit{\textbf{sum}} \\
\cmidrule{2-5}\textit{\textbf{bN}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{i}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\textit{\textbf{mul}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .4,  .761,  .643}.50 \\
\textit{\textbf{sum}} & \cellcolor[rgb]{ .929,  .973,  .984}0 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 & \cellcolor[rgb]{ .137,  .545,  .271}1 \\
\end{tabular}%


==> data/prof-347.tex <==
\small

% Table generated by Excel2LaTe$\vert$ from sheet '347'
\begin{tabular}[b]{ccccrrr}
\textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{mul}} & \textit{\textbf{sum}} &       &       &  \\
\cmidrule{1-4}\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{1}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{void convertBinArr(int[] bN)$\{$}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{2}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} int sum=0;}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{3}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} int mul=1;}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{4}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} for(int i=0;i$<$bN.length;i++)$\{$}} \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{5}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}ii\color{black} sum+=mul*bN[i];}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{6}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}ii\color{black} mul*=2;  $\}$}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{7}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} System.out.println(sum);}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{8}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} System.out.println(intToStr(sum/16)}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{r|}{} & \multicolumn{1}{l}{\texttt{\color{white}ii\color{black} +intToStr(sum\%16));$\}$}} \\
\cmidrule{1-4}\rowcolor[rgb]{ .137,  .545,  .271} 1     & 1     & .89   & 1     & \cellcolor[rgb]{ 1,  1,  1} & \cellcolor[rgb]{ 1,  1,  1} & \cellcolor[rgb]{ 1,  1,  1} \\
\end{tabular}%




==> data/slice-table1-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{cccc}
\textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{i}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} \\
\multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{r|}{} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\multicolumn{1}{r|}{} & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$ \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}B \\
\multicolumn{1}{r|}{} & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$ \\
\multicolumn{1}{r|}{} & \multicolumn{1}{r|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} &  \\
\midrule
\rowcolor[rgb]{ .4,  .761,  .643} .67   & \cellcolor[rgb]{ .137,  .545,  .271}.78 & \cellcolor[rgb]{ .929,  .973,  .984}.22 & \cellcolor[rgb]{ .137,  .545,  .271}.78 \\
\end{tabular}%


==> data/slice-table1-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{cccc}
\textit{\textbf{bN}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}F \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & $\vert$ $\vert$ $\vert$ \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}B \\
\midrule
\rowcolor[rgb]{ .137,  .545,  .271} 1     & 1     & .87   & 1 \\
\end{tabular}%


==> data/slice-table2-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}{ccccc}
\textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{hD}} & \textit{\textbf{i}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{} &  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$ \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}B \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & $\vert$ \\
\midrule
\rowcolor[rgb]{ .137,  .545,  .271} .79   & \cellcolor[rgb]{ .4,  .761,  .643}.50 & \cellcolor[rgb]{ .929,  .973,  .984}.07 & \cellcolor[rgb]{ .4,  .761,  .643}.71 & .86 \\
\end{tabular}%


==> data/slice-table2-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
\begin{tabular}{ccccc}
\textit{\textbf{bN}} & \textit{\textbf{c 1/2}} & \textit{\textbf{i}} & \textit{\textbf{m}} & \textit{\textbf{sum}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}F \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & $\vert$ $\vert$ $\vert$ \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F / } & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651} / F} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}B \\
\midrule
\rowcolor[rgb]{ .137,  .545,  .271} 1     & \cellcolor[rgb]{ .929,  .973,  .984}.10 & 1     & .90   & 1 \\
\end{tabular}%


==> data/slice-table3-25.tex <==
\small
% Table generated by Excel2LaTeX from sheet '25'
\begin{tabular}[t]{cccccc}
\textit{\textbf{bN}} & \textit{\textbf{dec}} & \multicolumn{2}{c}{\textit{\textbf{hex}}} & \textit{\textbf{hD 1/2}} & \textit{\textbf{i}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{} &  \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F / $\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}$\vert$ / F} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & $\vert$ $\vert$ $\vert$ & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$ \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}B \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}F & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & $\vert$ \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$ \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ .651,  .651,  .651}B & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & $\vert$ \\
\midrule
\rowcolor[rgb]{ .137,  .545,  .271} .75   & \cellcolor[rgb]{ .698,  .886,  .886}.44 & \multicolumn{2}{c}{\cellcolor[rgb]{ .698,  .886,  .886}.41} & .75   & .81 \\
\end{tabular}%


==> data/slice-table3-347.tex <==
\small
% Table generated by Excel2LaTeX from sheet '347'
% Table generated by Excel2LaTe$\vert$ from sheet '347'
\begin{tabular}[t]{rrrr}
\multicolumn{1}{c}{\textit{\textbf{bN}}} & \multicolumn{1}{c}{\textit{\textbf{i}}} & \multicolumn{1}{c}{\textit{\textbf{m}}} & \multicolumn{1}{c}{\textit{\textbf{sum}}} \\
\midrule
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{$\vert$} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{$\vert$} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
\midrule
\rowcolor[rgb]{ .137,  .545,  .271} \multicolumn{1}{c}{1} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{.89} & \multicolumn{1}{c}{1} \\
      &       &       &  \\
      &       &       &  \\
\end{tabular}%


==> data/student-25.tex <==
\small

% Table generated by Excel2LaTe$\vert$ from sheet '25'
\begin{tabular}[b]{ccccccrrr}
\textit{\textbf{bN}} & \textit{\textbf{dec}} & \textit{\textbf{hex}} & \textit{\textbf{hD1}} & \textit{\textbf{hD2}} & \textit{\textbf{i}} &       &       &  \\
\cmidrule{1-6}\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \cellcolor[rgb]{ 1,  1,  1} & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{1}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{void convertBinArr(}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{} & \multicolumn{1}{l}{\texttt{\color{white}ii\color{black} int[] bN)$\{$}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{\texttt{2}} & \multicolumn{1}{l}{\texttt{\color{white}i\color{black} double dec=0;}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}\_ / F} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{\texttt{3}} & \multicolumn{1}{l}{\texttt{\color{white}i\color{black} String hex="";}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ &       & \multicolumn{1}{r|}{\texttt{4}} & \multicolumn{1}{l}{\texttt{\color{white}i\color{black} double hD1=0;}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} &       &       & \multicolumn{1}{r|}{\texttt{5}} & \multicolumn{1}{l}{\texttt{\color{white}i\color{black} double hD2=0;}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \multicolumn{1}{c|}{$\vert$ $\vert$ $\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}F $\vert$ $\vert$ & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{6}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} for(int i = 0;}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{} & \multicolumn{1}{l}{\texttt{\color{white}iii\color{black} i$<$bN.length; i++)$\{$}} \\
\rowcolor[rgb]{ .651,  .651,  .651} \multicolumn{1}{c|}{B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851}$\vert$} & \cellcolor[rgb]{ .851,  .851,  .851}$\vert$ & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{7}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}ii\color{black} if(bN[i]$==$1)$\{$}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{8}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}iii\color{black} dec+=Math.pow(2,i);}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{9}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}iii\color{black} if(i$<=$3)}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{10}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}iiii\color{black} hD2+=Math.pow(2,i);}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{11}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}iii\color{black} if(i$>$3)}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & \cellcolor[rgb]{ .651,  .651,  .651}B & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{12}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}iiii\color{black} hD1+=Math.pow(2,i-4);}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{} & \multicolumn{1}{l}{\texttt{    $\}$  $\}$}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}F} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{13}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} hex=hexString(hD1)}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &       &       & \multicolumn{1}{r|}{} & \multicolumn{1}{l}{\texttt{\color{white}ii\color{black} +hexString(hD2);}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{14}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} System.out.println(dec);}} \\
\rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{\cellcolor[rgb]{ 1,  1,  1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .651,  .651,  .651}B} & \multicolumn{1}{c|}{$\vert$} & \multicolumn{1}{c|}{$\vert$} & $\vert$     & \cellcolor[rgb]{ 1,  1,  1} & \multicolumn{1}{r|}{\cellcolor[rgb]{ 1,  1,  1}\texttt{15}} & \multicolumn{1}{l}{\cellcolor[rgb]{ 1,  1,  1}\texttt{\color{white}i\color{black} System.out.println(hex);$\}$}} \\
\cmidrule{1-6}\rowcolor[rgb]{ .137,  .545,  .271} .75   & \cellcolor[rgb]{ .698,  .886,  .886}.44 & \cellcolor[rgb]{ .698,  .886,  .886}.41 & .75   & .75   & .81   & \cellcolor[rgb]{ 1,  1,  1} & \cellcolor[rgb]{ 1,  1,  1} & \cellcolor[rgb]{ 1,  1,  1} \\
\end{tabular}%




